Property {A} and duality in linear programming

Property A is a form of weak amenability for groups and metric spaces introduced as an approach to the famous Novikov higher signature conjecture, one of the most important unsolved problems in topology. We show that property A can be reduced to a sequence of linear programming optimization problems on finite graphs. We explore the dual problems, which turn out to have interesting interpretations as combinatorial problems concerning the maximum total supply of flows on a network. Using isoperimetric inequalities, we relate the dual problems to the Cheeger constant of the graph and explore the role played by symmetry of a graph to obtain a striking characterization of the difference between an expander and a graph without property A. Property A turns out to be a new measure of connectivity of a graph that is relevant to graph theory. The dual linear problems can be solved using a variety of methods, which we demonstrate on several enlightening examples. As a demonstration of the power of this linear programming approach we give elegant proofs of theorems of Nowak and Willett about graphs without property A.

==> introduction.tex <==
\section{Introduction}
Property A is a form of weak amenability for groups and metric spaces introduced by G.~Yu~\cite{yu2000} at the turn of the century as an approach to the famous Novikov higher signature conjecture. First stated over fifty years ago, the Novikov conjecture asserts that the so-called higher signatures determined by a discrete group $\Gamma$ are homotopy invariant and remains one of the most important unsolved problems in topology~\cite{frr1995}.

Yu proved that a discrete metric space $X$ with property A admits a coarsely uniform embedding into Hilbert space, which implies the coarse Baum-Connes conjecture, which (in the case that $X$ is the Cayley graph of a finitely generated group $\Gamma$) implies the Novikov conjecture for $\Gamma$. 

Property A is an invariant of coarse isometry. Among the spaces that have property A are spaces with finite asymptotic dimension~\cite{higson-roe2000} or spaces with finite decomposition complexity~\cite{guentner-tessera-yu2012}. Moreover property A is preserved by standard constructions such as products, unions, and group extensions among others~\cite{dydak-virk2016,guentner2014}.

Although several classes of graphs without property A are known to exist, the proofs that these graphs fail to have property A either rely on an obstruction to embedding in Hilbert space (as in the case of the so-called Gromov monster groups~\cite{gromov2003}) or rely on ad hoc methods. Indeed, prior to the examples constructed by P.~Nowak~\cite{nowak2007}, it was not clear what lay in the realm between property A and uniform embeddability in Hilbert space.

The aim of this paper is to leverage the power of duality theory in linear programming to characterize property A in a way that provides a means to detect when a graph fails to have property A in a unified way and in a way that does not rely on obstructing embedding into Hilbert space. Using this approach, we are able to show that: graphs that have a sequence of expanders fail to have property A~\cite{gromov2003}; Nowak's union of cubes fails to have property A~\cite{nowak2007}; and Willett's graphs with large girth fail to have property A~\cite{willett2011}.

Moreover, we are able to characterize the difference between a group having an expander in its Cayley graph and a group that fails to have property A. 

Property A is only interesting for infinite graphs and linear programming requires finite graphs. Therefore, we check our conditions on an increasing sequence of isometrically embedded subgraphs and show that this limit characterizes property A (for locally finite graphs). 

The main idea is to describe property A as a linear optimization problem that seeks a minimum variation on probability measures across edges of a graph. As in the usual property A, one finds a sequence of such probability measures whose differences approach $0$ to prove that the graph has property A. The novelty of our approach is that using duality theory, we can recast this (primal) optimization problem as a dual problem in which a quantity must be maximized. The duality theory tells us that an admissible solution to the dual problem bounds an admissible solution to the primal problem from below and the optimal solutions are equal. This means that if we can bound solutions to the dual problem away from $0$, we may conclude that there is no sequence of probability measures on an increasing family of graphs whose variation tends to $0$; i.e., the graph fails to have property A. 

The relationship between a primal and dual problem is rich and yields insight into different formulations of property A in terms of probability measures, partitions of unity, pseudo-flows, or isoperimetric inequalities, (see the top of  Figure~\ref{fig: primal and dual problems}). Moreover, we can fine tune these problems in interesting ways: for example, we may impose further restrictions on the dual problem, which amount to a relaxation of the conditions in the primal problem. It is in this way that we see that there is quite a bit of ``room'' between the notions of graphs containing a sequence of expanders and graphs that fail to have property A. This sort of analysis also opens new avenues of research. Among these, we explore ``mean property A'' but do not consider further primal problems that correspond to stricter conditions in the the dual realm, see Figure~\ref{fig: primal and dual problems}. 

The paper is arranged as follows. We begin by framing property~A for graphs at a fixed scale $\mathcal{S}$ as an optimization problem that is reminiscent of the definition of property~A for metric spaces in terms of existence of $\mathcal{S}$-supported probability measures with $(R,\epsilon)$ variation. This is then recast as a linear problem. Next, we construct the dual problem, which is a maximization problem, which can be understood in terms of a pseudo-flow on G.
Next, we remove the language of flows and instead express the dual problem in the language of a weighted isoperimetric inequality. We show that this (equivalent) formulation of the dual problem is dual to the well-known definition of property~A in terms of partitions of unity. 
\todo[inline]{Contents and main theorems of the paper here.}

%\textbf{OLD MATERIAL FOLLOWS.}
%
%Property A was introduced in~\cite{yu2000} and turns out to be of great
%importance in many areas of mathematics~\cite{nowak-yu2008}. Perhaps the most striking example is the following implication that follows from results in~\cite{yu2000}.
%
%\begin{quote}
%If a finitely generated group $G$ has property A then the Novikov conjecture is
%true for all closed manifolds with fundamental
%group $G$.
%\end{quote}
%The Novikov conjecture asserts homotopy invariance of higher signatures of smooth manifolds and is one of most important unsolved problems in topology.
%
%It is difficult to find an example of a finitely generated group without property~A.
%The only known methods use probability techniques to construct groups
%  that contain expanders in their Cayley graphs.
% The elusiveness of such examples motivates interest in invariants that imply that property~A fails.
%In the present paper we apply the strong duality theorem from linear programming to construct such invariants. 
%We also characterize the difference between a group having an expander in its Cayley graph and a group that fails to have property A.

{
% https://tex.stackexchange.com/questions/346106/creating-cube-with-tikz
% https://tex.stackexchange.com/questions/8890/tikz-how-to-draw-boxes-around-set-of-nodes
\tikzset{%
    node distance=15mm,
    lp/.style={
      rectangle,
      draw=gray,
      thick,
      fill=gray!20,
      text width=25mm,
      align=center,
      % rounded corners,
      minimum height=1cm
    },
    every node/.style={%
        align=center,
        fill=white,
        font=\small
    },
    every edge/.append style={every node/.style={font=\footnotesize, fill=white}}
}

\begin{figure}[t]%[H]
\begin{center}
\begin{tikzpicture}
\node (p) {\bf Primal Problems\\ (minimization)};
\node[right=28mm of p] (d) {\bf Dual Problems\\ (maximization)};

\node[lp, below=2cm of p.west, anchor=west] (p1) {Probability Measures (\ref{lp:measures})};
\node[lp, below right=2cm and -2mm of p1] (p2) {Partitions of Unity (\ref{lp:partition})};

\node[lp, below=2cm of d.west, anchor=west] (d1) {Pseudo Flows (\ref{lp:pseudo-flows})};
\node[lp, below right=2cm and 6mm of d1] (d2) {Isoperimetric Inequalities (\ref{lp:isoperimetric})};

\node[lp, below=80mm of p1] (p5) {Mean Property A};

\node[lp, below=35mm of d2] (d4) {Weighted Edge Expansion};
\node[lp, below=80mm of d1] (d5) {Uniform Flows};
\node[lp, below=35mm of d4] (d6) {Cheeger Constant};

\node[above left=1mm and 1mm of d] (sep top) {};
\node[below left=31mm and 1mm of d5] (sep bot) {};

\path (sep top) edge[dashed, draw=gray] (sep bot);

\path (p5) edge node[align=center] {$=$\\ Duality} (d5);
\path (p1) edge node[align=center] {$\geq$\\ Relaxation} (p5);

\path (p1) edge node[align=center] {$=$\\ Theorem~\ref{thm:measures equals partition}} (p2);
\path (p1) edge node[align=center] {$=$\\ Duality\\ Theorem~\ref{thm:duality}} (d1);
\path (d1) edge node[align=center] {$=$\\ Lift and Project\\ Theorem~\ref{thm:lift and project}} (d2);

\path (d1) edge node[align=center] {$\geq$\\ Fix $\eta_i = \eta$\\ Fix $\kappa_{ij} = \frac 1{|E|}$} (d5);

\path (d2) edge node[align=center] {$\geq$\\ Fix $\eta_i = \eta$} (d4);
\path (d4) edge node[align=center] {$\geq$\\ Fix $\kappa_{ij} = \frac 1{|E|}$} (d6);
\path (d5) edge node[align=center] {$=$\\ Lift and Project} (d6);

\path (p2) edge node[align=center, near end] {$=$\\ Duality\\ Lemma~\ref{lem:isoperimetric dual to partition}} (d2);

\end{tikzpicture}
\end{center}
\caption{This is what we have now and it might be enough.}
\label{fig: primal and dual problems}
\end{figure}
}

